The Random Walk of High Frequency Trading

This paper builds a model of high-frequency equity returns by separately modeling the dynamics of trade-time returns and trade arrivals. Our main contributions are threefold. First, we characterize the distributional behavior of high-frequency asset returns both in ordinary clock time and in trade time. We show that when controlling for pre-scheduled market news events, trade-time returns of the highly liquid near-month E-mini S&P 500 futures contract are well characterized by a Gaussian distribution at very fine time scales. Second, we develop a structured and parsimonious model of clock-time returns by subordinating a trade-time Gaussian distribution with a trade arrival process that is associated with a modified Markov-Switching Multifractal Duration (MSMD) model. This model provides an excellent characterization of high-frequency inter-trade durations. Over-dispersion in this distribution of inter-trade durations leads to leptokurtosis and volatility clustering in clock-time returns, even when trade-time returns are Gaussian. Finally, we use our model to extrapolate the empirical relationship between trade rate and volatility in an effort to understand conditions of market failure. Our model suggests that the 1,200 km physical separation of financial markets in Chicago and New York/New Jersey provides a natural ceiling on systemic volatility and may contribute to market stability during periods of extremely heavy trading.

==> introAdd.tex <==



==> x.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{Chen2013}
\citation{Chen2013}
\citation{Brogaard2013}
\citation{Hasbrouck2013}
\citation{Bachelier1900}
\citation{Black1973}
\citation{Fama1965}
\citation{Hasbrouck2003}
\citation{Bouchaud2005}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{2}{section.1}}
\newlabel{intro}{{1}{2}{Introduction}{section.1}{}}
\citation{Brada1966}
\citation{Mandelbrot1967}
\citation{Mandelbrot1963}
\citation{Clark1973}
\citation{Ane2000}
\citation{Chen2013}
\citation{Mandelbrot1997}
\citation{Calvet1997}
\citation{Fisher1997}
\citation{Calvet2001}
\citation{Calvet2002}
\citation{Calvet2004}
\citation{Ane2000}
\citation{Chen2013}
\citation{Laughlin2012}
\@writefile{toc}{\contentsline {section}{\numberline {2}Data}{4}{section.2}}
\newlabel{data}{{2}{4}{Data}{section.2}{}}
\citation{Laughlin2012}
\citation{Mandelbrot1963}
\citation{Engle1982}
\citation{Bollerslev1986}
\citation{Brada1966}
\citation{Mandelbrot1967}
\citation{Clark1973}
\citation{Ane2000}
\@writefile{toc}{\contentsline {section}{\numberline {3}Empirical Distributions of Intra-Day Asset Returns}{8}{section.3}}
\newlabel{distributions}{{3}{8}{Empirical Distributions of Intra-Day Asset Returns}{section.3}{}}
\newlabel{ctrets}{{1}{8}{Empirical Distributions of Intra-Day Asset Returns}{equation.3.1}{}}
\newlabel{ttrets}{{2}{8}{Empirical Distributions of Intra-Day Asset Returns}{equation.3.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Intra-day Clock-Time and Trade-Time Distributions}{8}{subsection.3.1}}
\citation{Gallant1992}
\citation{Aldrich2011}
\@writefile{toc}{\contentsline {section}{\numberline {4}Model}{12}{section.4}}
\newlabel{model}{{4}{12}{Model}{section.4}{}}
\newlabel{gaussTick}{{3}{12}{Model}{equation.4.3}{}}
\newlabel{mix}{{5}{12}{Model}{equation.4.5}{}}
\citation{Press1967}
\citation{Press1968}
\citation{Chen2013}
\citation{Calvet2001}
\citation{Calvet2002}
\citation{Calvet2004}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Compound Poisson Process}{13}{subsection.4.1}}
\newlabel{compPois}{{4.1}{13}{Compound Poisson Process}{subsection.4.1}{}}
\newlabel{mixPoisson}{{7}{13}{Compound Poisson Process}{equation.4.7}{}}
\citation{Chen2013}
\citation{Calvet2008}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Compound Multifractal Process}{14}{subsection.4.2}}
\newlabel{compMF}{{4.2}{14}{Compound Multifractal Process}{subsection.4.2}{}}
\newlabel{msmd}{{8}{14}{Compound Multifractal Process}{equation.4.8}{}}
\newlabel{msmd1}{{8a}{14}{Compound Multifractal Process}{equation.4.8a}{}}
\newlabel{msmd2}{{8b}{14}{Compound Multifractal Process}{equation.4.8b}{}}
\newlabel{msmd3}{{8c}{14}{Compound Multifractal Process}{equation.4.8c}{}}
\newlabel{msmd4}{{8d}{14}{Compound Multifractal Process}{equation.4.8d}{}}
\newlabel{msmd5}{{8e}{14}{Compound Multifractal Process}{equation.4.8e}{}}
\newlabel{msmd6}{{8f}{14}{Compound Multifractal Process}{equation.4.8f}{}}
\citation{Chen2013}
\citation{Chen2013}
\citation{Chen2013}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Compound Truncated Multifractal Process}{16}{subsection.4.3}}
\newlabel{compTMF}{{4.3}{16}{Compound Truncated Multifractal Process}{subsection.4.3}{}}
\newlabel{msmdExp}{{9}{16}{Compound Truncated Multifractal Process}{equation.4.9}{}}
\newlabel{msmdExp1}{{9a}{16}{Compound Truncated Multifractal Process}{equation.4.9a}{}}
\newlabel{msmdExp2}{{9b}{16}{Compound Truncated Multifractal Process}{equation.4.9b}{}}
\newlabel{msmdExp3}{{9c}{16}{Compound Truncated Multifractal Process}{equation.4.9c}{}}
\citation{Chen2013}
\citation{Chen2013}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4}Comparison of Duration Models}{17}{subsection.4.4}}
\newlabel{comparison}{{4.4}{17}{Comparison of Duration Models}{subsection.4.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {5}Estimation and Results}{18}{section.5}}
\newlabel{results}{{5}{18}{Estimation and Results}{section.5}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Poisson/Exponential Estimation}{19}{subsection.5.1}}
\newlabel{expEst}{{5.1}{19}{Poisson/Exponential Estimation}{subsection.5.1}{}}
\newlabel{expMean}{{10}{19}{Poisson/Exponential Estimation}{equation.5.10}{}}
\citation{Chen2013}
\citation{Hamilton1989}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Estimates (standard errors in parentheses) of component distribution parameters for $m=1$. For the MSMD and TMSMD models, $\mathaccentV {bar}016{k}= 7$.\relax }}{20}{table.caption.11}}
\newlabel{estimates}{{1}{20}{Estimates (standard errors in parentheses) of component distribution parameters for $m=1$. For the MSMD and TMSMD models, $\bar {k}= 7$.\relax }{table.caption.11}{}}
\newlabel{poisProc}{{11}{20}{Poisson/Exponential Estimation}{equation.5.11}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}MSMD Estimation}{20}{subsection.5.2}}
\newlabel{msmdEst}{{5.2}{20}{MSMD Estimation}{subsection.5.2}{}}
\citation{Chen2013}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces Likelihood values at the maximum likelihood estimates for various values of $\mathaccentV {bar}016{k}$ and for $m=1$.\relax }}{21}{table.caption.12}}
\newlabel{likevals}{{2}{21}{Likelihood values at the maximum likelihood estimates for various values of $\bar {k}$ and for $m=1$.\relax }{table.caption.12}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3}TMSMD Estimation}{21}{subsection.5.3}}
\newlabel{tmsmdEst}{{5.3}{21}{TMSMD Estimation}{subsection.5.3}{}}
\newlabel{maxdmaxExp}{{12}{22}{TMSMD Estimation}{equation.5.12}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.4}Trade-time Gaussian Estimation}{22}{subsection.5.4}}
\newlabel{gaussEst}{{5.4}{22}{Trade-time Gaussian Estimation}{subsection.5.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.5}Simulating Clock-time Returns}{23}{subsection.5.5}}
\newlabel{compEst}{{5.5}{23}{Simulating Clock-time Returns}{subsection.5.5}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces Number (fraction in parentheses) of simulated clock-time returns that were adjusted to fall within the support of discretely observed data values.\relax }}{24}{table.caption.14}}
\newlabel{threshhold}{{3}{24}{Number (fraction in parentheses) of simulated clock-time returns that were adjusted to fall within the support of discretely observed data values.\relax }{table.caption.14}{}}
\@writefile{lot}{\contentsline {table}{\numberline {4}{\ignorespaces Goodness of fit statistics for simulated returns under the Exponential and MSMD duration models. The first three rows report $\chi ^2$ goodness of fit measures relative to the observed data for each clock time interval $\tau $ that we consider. The latter three rows report Kullback-Leibler divergences, again, relative to the observed data.\relax }}{26}{table.caption.16}}
\newlabel{gofStats}{{4}{26}{Goodness of fit statistics for simulated returns under the Exponential and MSMD duration models. The first three rows report $\chi ^2$ goodness of fit measures relative to the observed data for each clock time interval $\tau $ that we consider. The latter three rows report Kullback-Leibler divergences, again, relative to the observed data.\relax }{table.caption.16}{}}
\@writefile{lot}{\contentsline {table}{\numberline {5}{\ignorespaces Ljung-Box statistics for simulated returns under the Exponential, MSMD and TMSMD duration models as well as the observed data for each clock time interval $\tau $ that we consider. The first four rows report Ljung-Box statistics for the ACFs of returns and the last four rows report Ljung-Box statistics for the ACFs of squared returns.\relax }}{28}{table.caption.19}}
\newlabel{lbStats}{{5}{28}{Ljung-Box statistics for simulated returns under the Exponential, MSMD and TMSMD duration models as well as the observed data for each clock time interval $\tau $ that we consider. The first four rows report Ljung-Box statistics for the ACFs of returns and the last four rows report Ljung-Box statistics for the ACFs of squared returns.\relax }{table.caption.19}{}}
\citation{Chen2013}
\@writefile{toc}{\contentsline {section}{\numberline {6}Conclusion}{29}{section.6}}
\newlabel{conclusion}{{6}{29}{Conclusion}{section.6}{}}
\@writefile{toc}{\contentsline {section}{\numberline {A}Expectation of the Maximum of Exponential Random Variables}{31}{appendix.A}}
\newlabel{extremum}{{A}{31}{Expectation of the Maximum of Exponential Random Variables}{appendix.A}{}}
\newlabel{extremeCDF}{{13}{31}{Expectation of the Maximum of Exponential Random Variables}{equation.A.13}{}}
\newlabel{extremePDF}{{14}{31}{Expectation of the Maximum of Exponential Random Variables}{equation.A.14}{}}
\newlabel{extremeExp}{{15}{31}{Expectation of the Maximum of Exponential Random Variables}{equation.A.15}{}}
\citation{*}
\bibstyle{asa}
\bibdata{newsDist}
\bibcite{Aldrich2011}{{1}{2013}{{Aldrich}}{{}}}
\bibcite{Ane2000}{{2}{2000}{{Ane and Geman}}{{}}}
\bibcite{Bachelier1900}{{3}{1900}{{Bachelier}}{{}}}
\bibcite{Black1973}{{4}{1973}{{Black and Scholes}}{{}}}
\bibcite{Bollerslev1986}{{5}{1986}{{Bollerslev}}{{}}}
\bibcite{Bouchaud2005}{{6}{2005}{{Bouchaud}}{{}}}
\bibcite{Brada1966}{{7}{1966}{{Brada et~al.}}{{Brada, Ernst, and van Tassel}}}
\bibcite{Brogaard2013}{{8}{2013}{{Brogaard et~al.}}{{Brogaard, Hendershott, and Riordan}}}
\bibcite{Calvet2001}{{9}{2001}{{Calvet and Fisher}}{{}}}
\bibcite{Calvet2002}{{10}{2002}{{Calvet and Fisher}}{{}}}
\bibcite{Calvet1997}{{11}{1997}{{Calvet et~al.}}{{Calvet, Fisher, and Mandelbrot}}}
\bibcite{Calvet2004}{{12}{2004}{{Calvet}}{{}}}
\bibcite{Calvet2008}{{13}{2008}{{Calvet and Fisher}}{{}}}
\bibcite{Calvet2012}{{14}{2012}{{Calvet and Fisher}}{{}}}
\bibcite{Chen2013}{{15}{2013}{{Chen et~al.}}{{Chen, Diebold, and Schorfheide}}}
\bibcite{Clark1973}{{16}{1973}{{Clark}}{{}}}
\bibcite{Easley2012}{{17}{2012}{{Easley et~al.}}{{Easley, de~Prado, and O'Hara}}}
\bibcite{Engle1982}{{18}{1982}{{Engle}}{{}}}
\bibcite{Fama1965}{{19}{1965}{{Fama}}{{}}}
\bibcite{Fisher1997}{{20}{1997}{{Fisher et~al.}}{{Fisher, Calvet, and Mandelbrot}}}
\bibcite{Gallant1992}{{21}{1992}{{Gallant et~al.}}{{Gallant, Rossi, and Tauchen}}}
\bibcite{Ghysels1995}{{22}{1995}{{Ghysels et~al.}}{{Ghysels, Gouri\'{e}roux, and Jasiak}}}
\bibcite{Hamilton1989}{{23}{1989}{{Hamilton}}{{}}}
\bibcite{Hasbrouck2003}{{24}{2003}{{Hasbrouck}}{{}}}
\bibcite{Hasbrouck2013}{{25}{2013}{{Hasbrouck and Saar}}{{}}}
\bibcite{Laughlin2012}{{26}{2012}{{Laughlin et~al.}}{{Laughlin, Aguirre, and Grundfest}}}
\bibcite{Mandelbrot1963}{{27}{1963}{{Mandelbrot}}{{}}}
\bibcite{Mandelbrot1997}{{28}{1997}{{Mandelbrot et~al.}}{{Mandelbrot, Fisher, and Calvet}}}
\bibcite{Mandelbrot1967}{{29}{1967}{{Mandelbrot and Taylor}}{{}}}
\bibcite{Mandelbrot1973}{{30}{1973}{{Mandelbrot}}{{}}}
\bibcite{Press1967}{{31}{1967}{{Press}}{{}}}
\bibcite{Press1968}{{32}{1968}{{Press}}{{}}}
\bibcite{Tauchen1983}{{33}{1983}{{Tauchen and Pitts}}{{}}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Time series plots of E-mini S\&P 500 futures contract prices for the 1000 seconds following 10:00 a.m. news announcements (red) and the 1000 seconds following 10:00 a.m. for a random selection of days without announcements (blue). Prices are all normalized by subtracting the initial price from all subsequent values. The upper panels show clock-time prices while the lower panels show trade-time prices. The legend reports selection dates and information on the individual news announcements.\relax }}{34}{figure.caption.1}}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{tsComp}{{1}{34}{Time series plots of E-mini S\&P 500 futures contract prices for the 1000 seconds following 10:00 a.m. news announcements (red) and the 1000 seconds following 10:00 a.m. for a random selection of days without announcements (blue). Prices are all normalized by subtracting the initial price from all subsequent values. The upper panels show clock-time prices while the lower panels show trade-time prices. The legend reports selection dates and information on the individual news announcements.\relax }{figure.caption.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Empirical density and Q-Q plots for clock-time and trade-time returns for both active and passive subsamples. The clock-time interval is $\tau = 10000$ milliseconds (10 seconds) and the trade-time interval is $m = 40$ (chosen to roughly match the clock-time interval).\relax }}{35}{figure.caption.2}}
\newlabel{qqHistComp}{{2}{35}{Empirical density and Q-Q plots for clock-time and trade-time returns for both active and passive subsamples. The clock-time interval is $\tau = 10000$ milliseconds (10 seconds) and the trade-time interval is $m = 40$ (chosen to roughly match the clock-time interval).\relax }{figure.caption.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Sample Q-Q plots for returns in both clock time and tick time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data. The vertical axes depict sample quantiles of the data and the horizontal axes depict theoretical quantiles of best-fit Gaussian distributions.\relax }}{36}{figure.caption.3}}
\newlabel{qqAll}{{3}{36}{Sample Q-Q plots for returns in both clock time and tick time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data. The vertical axes depict sample quantiles of the data and the horizontal axes depict theoretical quantiles of best-fit Gaussian distributions.\relax }{figure.caption.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Sample autocorrelation plots for returns in both clock time and trade time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data.\relax }}{37}{figure.caption.4}}
\newlabel{acAll}{{4}{37}{Sample autocorrelation plots for returns in both clock time and trade time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data.\relax }{figure.caption.4}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces Sample autocorrelation plots for squared returns in both clock time and trade time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data.\relax }}{38}{figure.caption.5}}
\newlabel{ac2All}{{5}{38}{Sample autocorrelation plots for squared returns in both clock time and trade time and in both active and passive subsamples. Each panel corresponds to a clock-time or trade-time interval during either the active or passive subsample of data.\relax }{figure.caption.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces A simulation of MSMD inter-trade durations for $\mathaccentV {bar}016{k} = 7$. The upper panels depict the time paths of latent states and MSMD rate parameter and the bottom panel depicts the durations themselves. This figure is a reproduction of Figure\nobreakspace  {}5 in \citet  {Chen2013}.\relax }}{39}{figure.caption.6}}
\newlabel{chenFig5}{{6}{39}{A simulation of MSMD inter-trade durations for $\bar {k} = 7$. The upper panels depict the time paths of latent states and MSMD rate parameter and the bottom panel depicts the durations themselves. This figure is a reproduction of Figure~5 in \citet {Chen2013}.\relax }{figure.caption.6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Histograms of simulated durations under the Exponential, MSMD and TMSMD models as well as observed inter-trade durations in the passive-period E-mini returns data.\relax }}{40}{figure.caption.7}}
\newlabel{durHist}{{7}{40}{Histograms of simulated durations under the Exponential, MSMD and TMSMD models as well as observed inter-trade durations in the passive-period E-mini returns data.\relax }{figure.caption.7}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces Quantile-Quantile plot. The vertical axis shows quantiles of simulated durations under the MSMD and TMSMD models and observed inter-trade durations in the passive-period E-mini returns data. The horizontal axis shows quantiles of simulated durations under the Exponential model. All model parameters are taken from Table\nobreakspace  {}\ref  {estimates}.\relax }}{41}{figure.caption.8}}
\newlabel{durQQ}{{8}{41}{Quantile-Quantile plot. The vertical axis shows quantiles of simulated durations under the MSMD and TMSMD models and observed inter-trade durations in the passive-period E-mini returns data. The horizontal axis shows quantiles of simulated durations under the Exponential model. All model parameters are taken from Table~\ref {estimates}.\relax }{figure.caption.8}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces Sample autocorrelation functions of simulated durations under the Exponential, MSMD and TMSMD models as well as observed inter-trade durations in the passive-period E-mini returns data.\relax }}{42}{figure.caption.9}}
\newlabel{durACF}{{9}{42}{Sample autocorrelation functions of simulated durations under the Exponential, MSMD and TMSMD models as well as observed inter-trade durations in the passive-period E-mini returns data.\relax }{figure.caption.9}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces Counting process distributions for $\tau = 10000$ ms. Each panel shows the counting distribution associated with one of the simulations (Exponential, MSMD and TMSMD), described in this section, overlaid with the empirical counting density of the passive-period E-mini returns. The simulations were obtained using the parameters estimates reported in Table\nobreakspace  {}\ref  {estimates}.\relax }}{43}{figure.caption.10}}
\newlabel{countingDens}{{10}{43}{Counting process distributions for $\tau = 10000$ ms. Each panel shows the counting distribution associated with one of the simulations (Exponential, MSMD and TMSMD), described in this section, overlaid with the empirical counting density of the passive-period E-mini returns. The simulations were obtained using the parameters estimates reported in Table~\ref {estimates}.\relax }{figure.caption.10}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces Profiles of the MSMD likelihood surface at the achieved maximum in the coordinate directions of the model parameters.\relax }}{44}{figure.caption.13}}
\newlabel{likeMap}{{11}{44}{Profiles of the MSMD likelihood surface at the achieved maximum in the coordinate directions of the model parameters.\relax }{figure.caption.13}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces Sample Q-Q plots for simulated clock-time returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TMSMD models (respectively), for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the E-mini passive-period clock-time Q-Q plots show in Figure\nobreakspace  {}\ref  {qqAll}.\relax }}{45}{figure.caption.15}}
\newlabel{simQQ}{{12}{45}{Sample Q-Q plots for simulated clock-time returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TMSMD models (respectively), for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the E-mini passive-period clock-time Q-Q plots show in Figure~\ref {qqAll}.\relax }{figure.caption.15}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces Sample autocorrelation functions for simulated clock-time returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TSMD models, for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the autocorrelations of E-mini passive-period clock-time returns in Figure\nobreakspace  {}\ref  {acAll}.\relax }}{46}{figure.caption.17}}
\newlabel{simAC}{{13}{46}{Sample autocorrelation functions for simulated clock-time returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TSMD models, for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the autocorrelations of E-mini passive-period clock-time returns in Figure~\ref {acAll}.\relax }{figure.caption.17}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {14}{\ignorespaces Sample autocorrelation functions for simulated clock-time \emph  {squared} returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TSMD models, for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the autocorrelations of E-mini passive-period clock-time squared returns in Figure\nobreakspace  {}\ref  {ac2All}.\relax }}{47}{figure.caption.18}}
\newlabel{simAC2}{{14}{47}{Sample autocorrelation functions for simulated clock-time \emph {squared} returns. The upper three rows of panels correspond to returns simulated under the Exponential, MSMD and TSMD models, for several clock time intervals $\tau $. The bottom row of panels is a reproduction of the autocorrelations of E-mini passive-period clock-time squared returns in Figure~\ref {ac2All}.\relax }{figure.caption.18}{}}

